The Cluster-EAGLE project: velocity bias and the velocity dispersion - mass relation of cluster galaxies

We use the Cluster-EAGLE simulations to explore the velocity bias introduced when using galaxies, rather than dark matter particles, to estimate the velocity dispersion of a galaxy cluster, a property known to be tightly correlated with cluster mass. The simulations consist of 30 clusters spanning a mass range $14.0 \le \log_{10}(M_{\rm 200c}/\mathrm{M_\odot}) \le 15.4$, with their sophisticated sub-grid physics modelling and high numerical resolution (sub-kpc gravitational softening) making them ideal for this purpose. We find that selecting galaxies by their total mass results in a velocity dispersion that is 5-10 per cent higher than the dark matter particles. However, selecting galaxies by their stellar mass results in an almost unbiased ($<5$ per cent) estimator of the velocity dispersion. This result holds out to $z=1.5$ and is relatively insensitive to the choice of cluster aperture, varying by less than 5 per cent between $r_{\rm 500c}$ and $r_{\rm 200m}$. We show that the velocity bias is a function of the time spent by a galaxy inside the cluster environment. Selecting galaxies by their total mass results in a larger bias because a larger fraction of objects have only recently entered the cluster and these have a velocity bias above unity. Galaxies that entered more than $4 \, \mathrm{Gyr}$ ago become progressively colder with time, as expected from dynamical friction. We conclude that velocity bias should not be a major issue when estimating cluster masses from kinematic methods.

==> OldTable.tex <==
% \begin{table*}
%     \centering
%     \caption{Best-fit parameters to the $\sigma_{\rm 200c}-M_{\rm 200c}$ relation for the DM particles and galaxies at $z=0$. Column~1 lists the simulation and sample details (with mass limits where appropriate). 
%     Column~2 gives the best-fit slope of the relation and the $1\sigma$ uncertainty. Columns 3-4 and 6-7 give the 
%     best-fit normalisation and scatter for a free and fixed slope respectively. Finally, columns 5 and 8 give the ratio of the 
%     normalisation to the case for DM particles, a measure of the velocity bias for the galaxies.}
%     \label{z0Params}
%     \begin{tabular}{l c c c c c c c c c}
%         \hline
%     \multicolumn{2}{c}{} & \multicolumn{3}{c}{$\alpha$ free} & \multicolumn{3}{c}{$\alpha=1/3$}\\
%          & $\alpha$ & $\sigma_{\mathrm{piv}} \, [\mathrm{km/s}]$ &  $\delta_{\ln} $ & $\sigma_\mathrm{piv}/\sigma_\mathrm{piv,DM}$ & $\sigma_{\mathrm{piv}} \, [\mathrm{km/s}] $ & 
%          $\delta_{\ln}$ & $\sigma_{\mathrm{piv}}/\sigma_{\mathrm{piv,DM}}$\\ 

%          \hline
    
%     C-EAGLE-DMO\\
%          DM Particles & $0.34 \pm 0.01$ & $805 \pm 8 $ & $0.048 \pm 0.006$ & & $803 \pm 7\phantom{0}$ & $0.048  \pm  0.006$\\ 

%          $M_\mathrm{Sub}:$ $10^9~-10^{10} \,  \mathrm{M_\odot}$ & $0.32 \pm 0.01$ & $887 \pm 7 $ & $0.035 \pm 0.005$ & $1.10 \pm 0.01$ &  $882 \pm 6\phantom{0}$ & $0.036  \pm  0.005$ & $1.10\pm0.01$\\ 

%          $M_\mathrm{Sub}:$ $10^{10}-10^{11} \, \mathrm{M_\odot}$ & $0.33 \pm 0.01$ & $893 \pm 7 $ & $0.033 \pm 0.004$ & $1.11 \pm 0.01$ & $891 \pm 6\phantom{0}$  & $0.035  \pm  0.005$ & $1.11\pm0.01$\\ 

%          $M_\mathrm{Sub}:$ $10^{11}-10^{12} \, \mathrm{M_\odot}$ & $0.33 \pm 0.02$ & $\phantom{0}894 \pm 13 $ & $0.062 \pm 0.008$ & $1.11 \pm 0.02$ & $891 \pm 10$  & $0.061  \pm  0.008$ & $1.11\pm0.02$\\

%          \hline

%     C-EAGLE-GAS\\
%          DM Particles & $0.35 \pm 0.01$ &  $804 \pm 9 $ & $0.055 \pm 0.007$ & & $800\pm9\phantom{0}$ & $0.058  \pm  0.007$\\ 

%          $M_\mathrm{Sub}:$ $10^9~-10^{10} \, \mathrm{M_\odot}$ & $0.32 \pm 0.01$ & $883 \pm 7 $ & $0.033 \pm 0.005$ & $1.10 \pm 0.01$ & $880\pm6\phantom{0}$ & $0.034  \pm  0.005$ & $1.10\pm0.01$\\ 

%          $M_\mathrm{Sub}:$ $10^{10}-10^{11} \, \mathrm{M_\odot}$ & $0.33 \pm 0.01$ & $885 \pm 8 $ & $0.034 \pm 0.004$ & $1.10 \pm 0.02$ & $883\pm6\phantom{0}$ & $0.035  \pm  0.004$ & $1.10\pm0.02$\\ 

%          $M_\mathrm{Sub}:$ $10^{11}-10^{12} \, \mathrm{M_\odot}$ & $0.34 \pm 0.02$ & $\phantom{0}844 \pm 11 $ & $0.08\phantom{0} \pm 0.01\phantom{0}$ & $1.05 \pm 0.02$ & $847\pm10$ & $0.09\phantom{0}  \pm  0.02\phantom{0}$ & $1.06\pm0.02$\\ 

%          %\hline

%          $M_{\mathrm{*}}\,\,\,\,\,:$ $10^{9~}-10^{10} \, \mathrm{M_\odot}$ & $0.32 \pm 0.02$ & $\phantom{0}823 \pm 11 $ & $0.06\phantom{0} \pm 0.01\phantom{0}$ & $1.02 \pm 0.02$ & $820\pm10$ & $0.062  \pm  0.007$ & $1.02\pm0.02$\\ 

%          $M_{\mathrm{*}}\,\,\,\,\,:$ $10^{10}-10^{11} \, \mathrm{M_\odot}$ & $0.36 \pm 0.02$ & $\phantom{0}789 \pm 13 $ & $0.11\phantom{0} \pm 0.02\phantom{0}$ & $0.98 \pm 0.02$ & $796\pm11$ & $0.11\phantom{0}  \pm  0.02\phantom{0}$ & $1.00\pm0.02$\\

%          \hline

%     \end{tabular}
% \end{table*}
